SupResDiffGAN a new approach for the Super-Resolution task

In this work, we present SupResDiffGAN, a novel hybrid architecture that combines the strengths of Generative Adversarial Networks (GANs) and diffusion models for super-resolution tasks. By leveraging latent space representations and reducing the number of diffusion steps, SupResDiffGAN achieves significantly faster inference times than other diffusion-based super-resolution models while maintaining competitive perceptual quality. To prevent discriminator overfitting, we propose adaptive noise corruption, ensuring a stable balance between the generator and the discriminator during training. Extensive experiments on benchmark datasets show that our approach outperforms traditional diffusion models such as SR3 and I$^2$SB in efficiency and image quality. This work bridges the performance gap between diffusion- and GAN-based methods, laying the foundation for real-time applications of diffusion models in high-resolution image generation.

==> figures/plots/prior_lpips.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[height=230pt, width = 450pt]{imgs/prior_lpips.png}
    \caption{Comparison of Interference Prior across different sizes of diffusion steps for SupResDiffGAN model  on CalebA-HQ, Imagenet and Urban100 datasets. Lpips metric.}
    \label{fig:prior_lpips}
\end{figure*}

==> figures/plots/steps_lpips.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{imgs/steps_lpips.png}
    \caption{Comparison of Diffusion Step Size of SupResDiffGAN model during interference on CalebA-HQ and Imagenet datasets. LPIPS metric.}
    \label{fig:steps_lpips}
\end{figure}

==> figures/plots/steps_ssim.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{imgs/steps_ssim.png}
    \caption{Comparison of Diffusion Step Size of SupResDiffGAN model during interference on CalebA-HQ and Imagenet datasets. SSIM metric.}
    \label{fig:steps_ssim}
\end{figure}

==> figures/plots/steps_time.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{imgs/steps_time.png}
    \caption{Comparison of Diffusion Step Size of SupResDiffGAN model during interference on CalebA-HQ and Imagenet datasets. Time per batch [s] metric.}
    \label{fig:steps_time}
\end{figure}
